LLM-TS Integrator: Integrating LLM for Enhanced Time Series Modeling

Time series~(TS) modeling is essential in dynamic systems like weather prediction and anomaly detection. Recent studies utilize Large Language Models (LLMs) for TS modeling, leveraging their powerful pattern recognition capabilities. These methods primarily position LLMs as the predictive backbone, often omitting the mathematical modeling within traditional TS models, such as periodicity. However, disregarding the potential of LLMs also overlooks their pattern recognition capabilities. To address this gap, we introduce \textit{LLM-TS Integrator}, a novel framework that effectively integrates the capabilities of LLMs into traditional TS modeling. Central to this integration is our \textit{mutual information} module. The core of this \textit{mutual information} module is a traditional TS model enhanced with LLM-derived insights for improved predictive abilities. This enhancement is achieved by maximizing the mutual information between traditional model's TS representations and LLM's textual representation counterparts, bridging the two modalities. Moreover, we recognize that samples vary in importance for two losses: traditional prediction and mutual information maximization. To address this variability, we introduce the \textit{sample reweighting} module to improve information utilization. This module assigns dual weights to each sample: one for prediction loss and another for mutual information loss, dynamically optimizing these weights via bi-level optimization. Our method achieves state-of-the-art or comparable performance across five mainstream TS tasks, including short-term and long-term forecasting, imputation, classification, and anomaly detection.

==> sections/introduction2.tex <==
\section{\tristan{Introduction 2 WIP Tristan, do not touch}}

Time series forecasting is a crucial task with broad applications across various fields including meteorology, economics, and industrial monitoring~\cite{hyndman2018forecasting, wu2021autoformer, friedman1962interpolation, gao2020robusttad, franceschi2019unsupervised}. Recent advancements have exploited Large Language Models (LLMs) for this purpose, due to their strong pattern recognition capabilities~\cite{jiang2024empowering, zhou2024one, jin2024timellm, sun2023test, gruver2024large, cao2023tempo}. This interest is driven by several factors: (1) the vast availability of textual data provides a robust training foundation for language models, generally enhancing their generalization capabilities; (2) the architectural similarities between models used for language and time series (both rely on sequence-based transformers), which have already shown promise in time series prediction~\cite{mirchandani2023large}; and (3) the potential for LLMs to impart few- and zero-shot learning capabilities to time series tasks, which could significantly extend the limited capabilities of existing time-series models in this area~\cite{radford2021learning, oreshkin2019n, oreshkin2020metalearning}.
\Sam{(1) is the point I mention in the original; (2) can be added; I think we should not mention (3) in case the reviewers challenge us as we do not have exps on few- and zero-shot.} \tristan{Yes, very good point Sam! In that case I'll think about how to replace that part with another argument.}
\Sam{(2) may not hold in our case as the main model we adopt in this paper is TimesNet, a CNN model.}

Despite apparent similarities between natural language and time series data, assuming that these extend to deeper functional similarities can be misleading. Traditional time series models typically utilize methods such as Fourier series and canonical decompositions to capture trends and seasonality~\cite{wu2021autoformer}, which are largely absent in LLM methodologies. Purely adapting language models risks omitting these domain-specific features, yet disregarding the potential of LLMs overlooks the aforementioned benefits. In response, we propose the \textit{LLM-TS Integrator}, a novel framework that enhances traditional time series forecasting with insights derived from LLMs through a mutual information maximization strategy.

The cornerstone of our approach is the \textit{mutual information} module, which augments a conventional predictive model, TimesNet~\cite{wu2023timesnet}, by integrating insights from LLMs. This integration aims to improve predictive accuracy while preserving the distinctive characteristics of time series data. By generating textual descriptions of time series data, we ensure maximal mutual information between these descriptions and the forecast outputs.

Moreover, our framework introduces a \textit{sample reweighting} module that adjusts the significance of individual samples based on their predictive and mutual information losses. This module utilizes a straightforward MLP network to assign dual weights to each sample, thereby optimizing information utilization throughout the model.

In summary, our primary contributions are:
\begin{itemize}
    \item The introduction of the LLM-TS Integrator framework, which uses mutual information to enhance time series modeling with LLM-derived capabilities.
    \item The development of a sample reweighting module that dynamically adjusts sample importance based on prediction and mutual information losses, thereby improving model efficiency.
    \item Comprehensive empirical validation across five key tasks, demonstrating our framework's effectiveness in enhancing time series forecasting.
\end{itemize}

